Nanomagnetic Self-Organizing Logic Gates

The end of Moore's law for CMOS technology has prompted the search for low-power computing alternatives, resulting in several promising proposals based on magnetic logic[1-8]. One approach aims at tailoring arrays of nanomagnetic islands in which the magnetostatic interactions constrain the equilibrium orientation of the magnetization to embed logical functionalities[9-12]. Despite the realization of several proofs of concepts of such nanomagnetic logic[13-15], it is still unclear what the advantages are compared to the widespread CMOS designs, due to their need for clocking[16, 17] and/or thermal annealing [18,19] for which fast convergence to the ground state is not guaranteed. In fact, it seems increasingly evident that "beyond CMOS" technology will require a fundamental rethinking of our computing paradigm[20]. In this respect, a type of terminal-agnostic logic was suggested[21], where a given gate is able to "self-organize" into its correct logical states, regardless of whether the signal is applied to the traditional input terminals, or the output terminals. Here, we introduce nanomagnetic self-organizing balanced logic gates, that employ stray-field coupled nanomagnetic islands to perform terminal-agnostic logic. We illustrate their capabilities by implementing reversible Boolean circuitry to solve a two-bit factorization problem via numerical modelling. In view of their design and mode of operation, we expect these systems to improve significantly over those suggested in Ref.[21], thus offering an alternative path to explore memcomputing, whose usefulness has already been demonstrated by solving a variety of hard combinatorial optimization problems[22].

==> Sections/07_contributions.tex <==
Must include all authors, identified by initials, for example:
A.A. conceived the experiment(s),  A.A. and B.A. conducted the experiment(s), C.A. and D.A. analysed the results.  All authors reviewed the manuscript. 


==> Sections/08_additionalInfo.tex <==
To include, in this order: \textbf{Accession codes} (where applicable); \textbf{Competing interests} (mandatory statement). 

The corresponding author is responsible for submitting a \href{http://www.nature.com/srep/policies/index.html#competing}{competing interests statement} on behalf of all authors of the paper. This statement must be included in the submitted article file.

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{stream}
\caption{Legend (350 words max). Example legend text.}
\label{fig:stream}
\end{figure}

\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|}
\hline
Condition & n & p \\
\hline
A & 5 & 0.1 \\
\hline
B & 10 & 0.01 \\
\hline
\end{tabular}
\caption{\label{tab:example}Legend (350 words max). Example legend text.}
\end{table}

Figures and tables can be referenced in LaTeX using the ref command, e.g. Figure \ref{fig:stream} and Table \ref{tab:example}.


==> Sections/Scaling.tex <==
After EC time (ranging from 10 ps to 160 ps), the logical consistency of an individual gate is checked. If necessary, static EC fields are applied during 10 ps to enforce the magnetic interaction and to quickly escape from a mete-stable non-logical state.\\
These EC fields can be realized with spin currents.

\subsection{AFW}
The anti-ferromagnetic wire (AFW) was constructed as a chain of NOT gates: the output of a NOT gate acts as the input of the next one. This means that each island belongs to 2 NOT gates (expect for the first and last island of the chain). In this way, each island only feels the magnetic stray field of its 2 nearest neighbours.\\
Without error correcting, starting from an initial state in which all islands having $m_z = -1$, the time to reach the ground state scales exponentially with the number of islands $N$ in the chain (Figure \ref{fig:EC_time}, red line).

\begin{figure}[H]
	\centerline{\includegraphics[width=3in]{Figures/EC_time.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:EC_time}
\end{figure}

\begin{figure}[H]
	\centerline{\includegraphics[width=3in]{Figures/EC_strength_tres.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:EC_strength}
\end{figure}

By applying EC fields, the scaling trend becomes polynomial for $N < 40$. This can be explained by Figure \ref{fig:Cor_EC_gnu}, which shows that the correlation length is increased with increasing EC time. For EC time = 10 ps, a local group of approximately 20 islands is formed giving rise to a polynomial scaling.


\begin{figure}[H]
	\centerline{\includegraphics[width=4in]{Figures/Cor_EC_gnu.png}}
	\caption{{\footnotesize BlaBla. }}
	\label{fig:Cor_EC_gnu}
\end{figure}

The EC strength can extend the amount of islands in the local group. However, these EC strengths correspond to current densities of $j_z \approx \frac{\beta M_s e d}{\overline{h}} =  10^{13}$ A/m$^2$ with $\beta$ the external (EC-)field and $d$ the free layer thickness which we assumed to be 10 nm. \textcolor{blue}{CHECK}
\begin{figure}[H]
	\centerline{\includegraphics[width=5in]{Figures/Cor_ECstrength_gnu.png}}
	\caption{{\footnotesize EC strength = 0.40 corresponds to an external field of 1 T which can be realized with a current density of 10$^{13}$ A/m$^2$.}}
	\label{fig:Cor_ECstrength_gnu}
\end{figure}


\subsection{Error correcting concept}
%\subsection{Slonczewski torque}
\textcolor{green}{Bartel?}

==> Sections/Suppl_DynamicalAnalysis.tex <==
We will simulate the sLLG dynamics (\ref{eq:sLLG}) of each proposed NAND gate design following two distinct protocols to evaluate consistency. The first protocol, which we will term {\it free-floating}, will allow the gates to evolve under the combined effects of thermal noise, magnetic interactions and no applied currents such that each non-fixed island magnetization will randomly switch as a result of these processes. We will assign (or not) a logical label $\lambda_q$ to the gate by observing the sign of the terminal island's perpendicular magnetization components at each moment in time. This allows us to compute the time spent by the gate in each allowed logical state and, as a result, estimate both $LC$ and $WB$. The second protocol, which we will term {\it clocked}, will periodically apply an in-plane polarized current pulse to each island to effectively reset all non-fixed islands and successively allowing them to relax again. The relaxation timescale setting the current periodicity is chosen to be smaller than the average switching timescale observed in the first protocol. At the end of each clocking cycle we assign a logical label to the gate's state and collect $LC$/$WB$ statistics over a large number of repetitions. This second protocol more closely emulates previous NML experiments where clocking fields are used to force gates to reset their magnetic states. The choice of these two protocols is two-fold. The first will assess gate robustness to successive spin-flip events while the second will assess robustness on individual relaxation events.

Figures~\ref{fig:DynOptimalA},~\ref{fig:DynOptimalB}, and ~\ref{fig:DynOptimalC} show the results obtained from the simulation of these two protocols. What immediately stands out is how the logical Boltzmann probabilities and, consequently, $LC$/$WB$ measures are very different from those obtained through the statical analysis of the previous section. This demonstrates how influential the evolution of the stray-fields as a result of dynamical transients can be. More specifically, the effectiveness of thermal noise at precluding the individual islands from ever exactly being in an $m_{i,z}=\pm 1$ state strongly invalidates expectations from the previous section. The results shown can however be considered significantly useful in the sense that both protocols produce statistics which are in strong agreement.   

\begin{figure}
	\centerline{\includegraphics[width=6in]{Figures/7_DynOptimalA.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:DynOptimalA}
\end{figure} 

\begin{figure}
	\centerline{\includegraphics[width=6in]{Figures/8_DynOptimalB.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:DynOptimalB}
\end{figure} 

\begin{figure}
	\centerline{\includegraphics[width=6in]{Figures/9_DynOptimalC.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:DynOptimalC}
\end{figure} 

We proceed nonetheless to consider the the effect of finely tuning the saturation magnetization $M_S$ of the free islands. Figures~\ref{fig:MsDynOptimalA} and \ref{fig:RevMsDynOptimalA} show how the observed logical probabilities are effected as a function of a scaling parameter multiplying $M_S$ in Eq. (\ref{eq:sLLG}) in the free-floating state. Figure~\ref{fig:MsDynOptimalA} considers a gate where the terminal islands are allowed to evolve freely whereas Figure~\ref{fig:RevMsDynOptimalA} constrains the output island into a $1$-state and monitors how the input islands respond. In both cases, the introduction of this new design flexibility allows to significantly boost both the $LC$ measure and control dispersion in the probability of the individual logical states. We do observe however that the optimal scaling factors are differ significantly between the constrained (Fig.~\ref{fig:MsDynOptimalA}) and unconstrained (Fig.~\ref{fig:RevMsDynOptimalA}) cases. Whereas the former displays optimal operation in accordance with a slight reduction of the free-island $M_S$, the latter displays optimality in the presence of a slight increase of the same. Nonetheless, we claim that this approach demonstrates that sufficient magnetic tunability exists to optimize the logical operation of stray-field-coupled NML gates when exposed to strong thermal effects exciting persistent out-of-equilibrium transient states.

\begin{figure}
	\centerline{\includegraphics[width=6in]{Figures/10_Ms_DynOptimalA.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:MsDynOptimalA}
\end{figure} 

\begin{figure}
	\centerline{\includegraphics[width=6in]{Figures/11_Reverse_Ms_DynOptimalA.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:RevMsDynOptimalA}
\end{figure} 



==> Sections/Suppl_ErrorSuppressionDetails.tex <==
\subsection{DES model}
The logical correctness is checked after a time $\tau_{\mathrm{check}}$ and, in case of a logically incorrect state, an additional field is applied on each island for a duration of $\tau_{\mathrm{DES}}$. This $\tau_{\mathrm{DES}}$ was chosen as fraction of average switching time of a gate with the ES field applied. For our parameters, this average switching time was 200~ps and $\tau_{\mathrm{DES}}=0.05\tau_{\mathrm{switch}}=$~10~ps. The rate a witch the logic is checked was set to $\tau_{\mathrm{check}}=4\tau_{\mathrm{DES}}=$~40~ps.

For a NAND and NOR gate consisting of input islands A and B, and output island C, these ES field were set at
\begin{eqnarray}
    B_{ES}^{A}(\mathrm{T}) &=& -0.080\bigg[ m_z^B/(\sqrt{3})^3 + m_z^C \bigg]\\
    B_{ES}^{B}(\mathrm{T}) &=& -0.080\bigg[ m_z^A/(\sqrt{3})^3 + m_z^C \bigg]\\
    B_{ES}^{C}(\mathrm{T}) &=& -0.080\bigg[ m_z^A + m_z^B \bigg] \pm 0.049
    \label{eq:ES_nandnor}
\end{eqnarray}
where the $+$sign and $-$sign of Eq.\ (\ref{eq:ES_nandnor}) correspond to the NAND and NOR gate, respectively. $m_z$ denotes the magnetization along the easy axis. The factor $(\sqrt{3})^3$ takes into account that magnetostatic interaction between the input islands is weaker due to the larger distance between these islands as shown in Figure \ref{fig:1_nand_design}(b). For a coupling between islands D and E, these ES field were set at 
\begin{eqnarray}
    B_{ES}^{D}(\mathrm{T}) &=& +0.080\ m_z^E\\
    B_{ES}^{E}(\mathrm{T}) &=& +0.080\ m_z^D
    \label{eq:ES_coup}
\end{eqnarray}
to promote that the magnetization of these islands points in the same direction. 

For a gate consisting of non-interacting islands, for which the logical NAND behavior is totally embedded within the ES scheme, these ES field were set at
\begin{eqnarray}
    B_{ES}^{A}(\mathrm{T}) &=& -0.080\bigg[ m_z^B/(\sqrt{3})^3 + m_z^C \bigg]+0.945H_{{\rm 2sm}}\\
    B_{ES}^{B}(\mathrm{T}) &=& -0.080\bigg[ m_z^A/(\sqrt{3})^3 + m_z^C \bigg]+0.945H_{{\rm 2sm}}\\
    B_{ES}^{C}(\mathrm{T}) &=& -0.080\bigg[ m_z^A + m_z^B \bigg] + 0.038 + 0.945\times2H_{{\rm 2sm}}
    \label{eq:ES_random}
\end{eqnarray}
with $H_{{\rm 2sm}} = 0.019 T$ the bias field obtained from the two-state model. For a coupling between non-interacting islands D and E, these ES field were set at 
\begin{eqnarray}
    B_{ES}^{D}(\mathrm{T}) &=& +0.640\ m_z^E\\
    B_{ES}^{E}(\mathrm{T}) &=& +0.640\ m_z^D.
    \label{eq:ES_randcoup}
\end{eqnarray}

\begin{figure}[H]
	\centerline{\includegraphics[width=\textwidth]{Figures/DES_paperSuppl5.png}}
	\caption{{\footnotesize {\bf Schematic representation of dynamic error suppression (DES).} {\bf (a)} $\tau_{\mathrm{DES}}$ = 4 $\tau_{\mathrm{on}}$ {\bf (b)} $\tau_{\mathrm{DES}}$ = $\tau_{\mathrm{on}}$.
	}}
	\label{fig:DES}
\end{figure}

\subsection{Coupling between gates}
\jonathan{Pieter?}

\subsection{Possible physical implementation}
Such a DES scheme could be realized by adding an extra hardware layer to the magnetic gate. The state of the nanomagnets can be read out through a magnetic tunnel junction (MTJ) and forward logic can be used detect the incorrect state and drive a correction signal in the form of a spin polarized current to help the incorrectly aligned magnets switch to a logically correct state. A lower power alternative could by realized by making use of voltage controlled magnetic anisotropy (VCmA)\cite{MAR-09,WEI-07} to increase the switching probability of the logical inconsistent island during the $\tau_{\mathrm{DES}}$.


==> Sections/Suppl_FixedOutput.tex <==
Due to the additional degrees of freedom of the macrospin model as compared to the two-state model, the magnetic moment of the bias island has to be tuned in order to recover the balancedness. The tuning of the relative bias was shown in Fig. 1(d) for a NAND gate with a free output. However, gates with a fixed output are required for solving factorization problems, i.e.\ to decompose a \emph{fixed} output number into its (prime)factors. Fixing the output affects the state space, which results in another tuning of the relative bias field (see Fig. \ref{fig:fixedout}).

The probability distributions of a SO-NAND gate and a SO-XNOR gate with fixed output are shown in Fig. \ref{fig:fixedout}(b) and (c), respectively. 

\begin{figure}[H]
	\centerline{\includegraphics[width=5in]{Figures/FixedOutput_paperSuppl.png}}
	\caption{{\footnotesize {\bf SO-gates with a fixed output.} {\bf (a)} The balancedness of a SO-NAND gate with output $1$ is recovered at a relative bias strength of 1.04, corresponding to the point where the probabilities of all logically correct states are equal, as indicated by the arrow. The two-state model corresponds to relative bias = 1. {\bf (b)} Probability distributions of a SO-NAND gate with fixed output {\bf (c)} Probability distributions of a SO-XNOR gate with fixed output.}}
	\label{fig:fixedout}
\end{figure}

==> Sections/Suppl_Influence.tex <==
As compared to the results of the two-state model, the  additional degrees of freedom in the macrospin model negatively impact the balancedness of the gate.

The balancedness can be recovered by tuning the magnetic moment of the bias island, as shown in Fig. 
 \ref{fig:1_nand_design}(d).
 Figure \ref{fig:influence}, shows that this tuning is robust as a $20\%$ change in the damping,  temperature, or uniaxial anisotropy constant of our system only result in a 2\% change of the required bias to recover the balancedness. 


\begin{figure}[H]
	\centerline{\includegraphics[width=\textwidth]{Figures/Tuning5.png}}
	\caption{{\footnotesize 
	Probabilities for the logic states, obtained with the macrospin model for different relative bias strengths for varying \textbf{(a)} damping, \textbf{(b)} temperature, and \textbf{(c)} anisotropy constant. The highlighted region corresponds to the simulation parameters of the main paper.}}
	\label{fig:influence}
\end{figure}



==> Sections/Suppl_NoteOnP-BitScaling.tex <==
As mentioned in the main text, the p-bit prime factorization demonstration~\cite{borders2019integer} required that the magnetic state of every sMTJ be read via magnetoresistive measurements on a timescale which scales inversely proportionately to the number of islands one wishes to have coupled. Assuming a network of $N$ coupled elements of which a subset $N_T$ is used to define the binary inputs one wishes to solve for~\footnote{In the case of a sum factorization operation attempting to obtain all pairs of 3-bit numbers whose sum is consistent with a given 4-bit output one must necessarily have $N\geq 6$ as at least one sMTJ is needed to represent each significant bit of the operation. In such a setting one would accordingly have $N_T=6$.}, the dynamics of the system must perform a Gibbs sampling of $2^{N_T}$ possible input states. Due to the exponential scaling of such a solution space, one must engineer for rapidly fluctuating sMTJ elements whose natural switching timescale $\tau_{\mathrm{switch}}$ is such that, relative to the maximum total operation time $\tau_{\mathrm{tot}}$ one has at disposal, the condition $\tau_{\mathrm{tot}}/\tau_{\mathrm{switch}}\gg 2^{N_T}/N_T$ holds. The origin of the $1/N_T$ contribution to the scaling results from the notion that the switching probability of any one free element can be roughly considered Poisson-distributed with mean switching time $\tau_{\mathrm{switch}}/N_T$. 

The number $N$ of free sMTJ elements used in such a construction can in principle be larger than $N_T$ depending on how the current biasings are constructed to define the Boolean problem of interest. This means that the intermediate three-step operation of magnetoresistive state read, digital elaboration of the biasing current intensities, and their application, must take place on a timescale $\tau_{\mathrm{adjust}} \ll \tau_{\mathrm{switch}}/N$ to ensure proper performance. To quantify the magnitude of these limitations, let us assume a natural sMTJ switching time of $\tau_{\mathrm{switch}}\simeq 1,\mu\mathrm{s}$ whose read/adjust operation can somehow be performed on a nanosecond timescale. Let us further assume that the Boolean problem of interest is ideally constructed ($N=N_T$). This places the fundamental limit $N_T\ll\tau_{\mathrm{switch}}/\tau_{\mathrm{adjust}}\sim 10^3 $ on the amount of significant bits one can operate on. One can of course engineer the sMTJ elements to have even slower natural switching times. For $\tau_{\mathrm{switch}}\sim 10\,\mu\mathrm{s}$ one might attempt to execute the reversion of an elliptic curve encryption operation by taking a public key as a fixed output and solving for its 256-bit private key pair. The total time taken to perform such an operation can be estimated, resulting in a gargantuan $\tau_{\mathrm{tot}}\simeq (2^{256}/256)\tau_{\mathrm{switch}}\sim 10^{69}\mathrm{s}$.)

==> Sections/Suppl_StaticAnalysis.tex <==

Logic gates are defined by their truth tables consisting of $\lambda_q,\,q=1,...,2^{N_{\mathrm{in}}}$ allowed combinations of simultaneous input/output terminal states. We will denote the set of allowed logical combinations as $\Lambda$. By fixing a certain logical function we wish to reproduce, at each iteration of terminal island labels we can assign an overall logical label $\lambda_s$ to each spin-flip state $\sigma_s$ if the magnetic state of the terminal island magnetizations replicates one of the input-output conditions defined by the logic function one is trying to emulate. Otherwise we will say that $\sigma_s\notin\Lambda$. The logical consistency $LC$ of the island configuration and terminal permutation chosen can then be defined as:

\begin{equation}
LC \equiv \frac{\sum_{s || \sigma_s\in\Lambda}\exp^{-\beta \epsilon(\sigma_s)}}{\sum_s \exp^{-\beta \epsilon(\sigma_s)}}.
\end{equation}  

Similarly we can compute the relative Boltzmann probability of all $\sigma_s$ spin-flip states satisfying a specific logical condition $\lambda_q$:

\begin{equation}
P[\lambda_q] = \frac{\sum_{s || \lambda_s=\lambda_q}\exp^{-\beta \epsilon(\sigma_s)}}{\sum_s \exp^{-\beta \epsilon(\sigma_s)}}.
\end{equation}
Well-Balancedness $WB$ can then be defined as the variance of the Boltzmann-averaged probabilities across all logical conditions:

\begin{equation}
WB \equiv \mathrm{var}(\{P[\lambda_q]\}).
\end{equation}

For NAND logic, where four distinct three-terminal combination are allowed out of a total of eight (see Table -reference-), it will always be the case that in the limit of large temperatures ($\beta\ll\epsilon(\sigma_{2^{(N-N_{\mathrm{fix}})}})$) $LC = 0.5$ and $WB = 0$. This must necessarily be so as in such a limit all terminal island combinations are equally likely ($P[\lambda_q]=0.125\;\forall q$). We wish to find gate configurations that maximize $LC$ while keeping $WB$ minimal across as wide a thermal energy range as possible. In Figure~\ref{fig:TriGate}, a simple gate design is used to highlight the temperature dependence of $LC$ and $WB$ on thermal energy. The gate highlights an example of a sub-optimal gate due to the fact that though it retains relatively high $LC$ values across an initial range of thermal energies, the Boltzmann probabilities of the individual logically allowed states are spread across a wide range throughout the range.

\begin{figure}[H]
	\centerline{\includegraphics[width=6in]{Figures/3_SimpleTriGate.png}}
	\caption{{\footnotesize Simple NAND gate design highlighting the typical dropoff of logical consistency and lowering of well-blanacedness as a function of increasing temperature. This gate would not be considered a good gate design due to the wide disparity of Boltzmann probabilities among the different logically allowed terminal island states. The table lists all eight possible spin-flip states $\sigma_s$ along with their respective logical labels and their relative energies.}}
	\label{fig:TriGate}
\end{figure} 

The three best performing gates obtained from our brute force search are shown in Figures~\ref{fig:OptimalA},~\ref{fig:OptimalB}, and~\ref{fig:OptimalC}. As expected, the $LC$ values drop off at high thermal energies for all of them. A significant thermal range exists, however, where values of $LC>0.75$. The gate designs proposed exhibit an exceptional balancedness due to the Boltzmann probabilities of each allowed logical state effectively equaling each other even though the ensembles rarely ever exhibit a degeneracy of states like the well-balanced gate mentioned in Section~2. Having massively narrowed down our search to these three potential NAND gate designs, we proceeded to study each dynamically to assess whether these static results hold in the presence of thermal excitations.


\begin{figure}[H]
	\centerline{\includegraphics[width=6in]{Figures/4_OptimalA.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:OptimalA}
\end{figure} 

\begin{figure}[H]
	\centerline{\includegraphics[width=6in]{Figures/5_OptimalB.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:OptimalB}
\end{figure} 

\begin{figure}[H]
	\centerline{\includegraphics[width=6in]{Figures/6_OptimalC.png}}
	\caption{{\footnotesize BlaBla.}}
	\label{fig:OptimalC}
\end{figure} 





